The Achilles' Heel of LLMs: How Altering a Handful of Neurons Can Cripple Language Abilities

Large Language Models (LLMs) have become foundational tools in natural language processing, powering a wide range of applications and research. Many studies have shown that LLMs share significant similarities with the human brain. Recent neuroscience research has found that a small subset of biological neurons in the human brain are crucial for core cognitive functions, which raises a fundamental question: do LLMs also contain a small subset of critical neurons? In this paper, we investigate this question by proposing a Perturbation-based Causal Identification of Critical Neurons method to systematically locate such critical neurons in LLMs. Our findings reveal three key insights: (1) LLMs contain ultra-sparse critical neuron sets. Disrupting these critical neurons can cause a 72B-parameter model with over 1.1 billion neurons to completely collapse, with perplexity increasing by up to 20 orders of magnitude; (2) These critical neurons are not uniformly distributed, but tend to concentrate in the outer layers, particularly within the MLP down\_proj components; (3) Performance degradation exhibits sharp phase transitions, rather than a gradual decline, when these critical neurons are disrupted. Through comprehensive experiments across diverse model architectures and scales, we provide deeper analysis of these phenomena and their implications for LLM robustness and interpretability. These findings can offer guidance for developing more robust model architectures and improving deployment security in safety-critical applications. Our code is available at https://github.com/qqqqqqqzx/The-Achilles-Heel-of-LLMs.

==> 3-Preliminary.tex <==









%This decomposition reveals that perplexity reflects three fundamental capabilities:

%\emph{Local Prediction Capability}: The model's ability to predict immediate token sequences based on short-range dependencies and statistical patterns, essential for basic text generation.

%\emph{Syntactic Understanding}: The model's grasp of grammatical structures and syntactic well-formedness, critical for instruction following and structured reasoning tasks.

%\emph{Semantic Coherence}: The model's capacity for maintaining topical consistency and logical reasoning, fundamental for knowledge retrieval, reading comprehension, and complex reasoning tasks.

%The cascading effect of language capability breakdown justifies perplexity as a predictor of downstream task failure. When critical neurons are disrupted, the resulting degradation in these core capabilities propagates to all dependent tasks. For instance, impaired syntactic understanding directly affects mathematical reasoning ability, while semantic coherence breakdown compromises knowledge retrieval tasks and reading comprehension. The exponential nature of perplexity amplifies even localized capability losses, making it highly sensitive to critical neuron disruptions and predictive of comprehensive task failure.




% To address the limitations identified in existing approaches, we establish mathematical definitions and measurement protocols that enable reproducible investigation of critical neuron dependencies. Our framework consists of three components: perplexity-based performance measurement, neuron masking interventions, and formal characterization of model collapse.

% \subsection{Perplexity Measurement}

% For a given input sequence $\mathbf{x} = (x_1, x_2, \ldots, x_T)$ with $T$ tokens, the perplexity of a language model $M$ is defined as the exponentiated average negative log-likelihood \citep{pascual-etal-2021-plug-play}:

% \begin{equation}
% \text{PPL}_M(\mathbf{x}) = \exp\left(-\frac{1}{T} \sum_{t=1}^{T} \log P_M(x_t | \mathbf{x_{<t}})\right)
% \end{equation}

% where $P_M(x_t | \mathbf{x_{<t}})$ denotes the probability assigned by model $M$ to token $x_t$ conditioned on the preceding context $\mathbf{x_{<t}} = (x_1, \ldots, x_{t-1})$.

% To understand how perplexity reflects multiple model capabilities, we decompose the conditional probability using the chain rule and information theory \citep{Shannon1948}. The log-likelihood term can be decomposed as:
% \begin{align}
% \log P_M(x_t | \mathbf{x_{<t}}) &= \log P_M(x_t | \mathbf{x_{<t}}, \mathcal{C}_t) + \log P_M(\mathcal{C}_t | \mathbf{x_{<t}}) \nonumber\\
% &= \underbrace{\log P_M(x_t | \mathcal{L}_t, \mathcal{S}_t)}_{\text{Local Prediction}} + \underbrace{\log P_M(\mathcal{L}_t | \mathbf{x_{<t}})}_{\text{Syntactic Understanding}} + \underbrace{\log P_M(\mathcal{S}_t | \mathbf{x_{<t}})}_{\text{Semantic Coherence}} 
% \end{align}

% where $\mathcal{C}_t$ represents the contextual information at position $t$, which we further decompose into:
% \begin{itemize}
% \item $\mathcal{L}_t$: Local linguistic patterns (n-gram dependencies, morphological constraints)
% \item $\mathcal{S}_t$: Semantic coherence requirements (topic consistency, discourse relations)
% \end{itemize}

% Substituting this decomposition into the perplexity formula yields:
% \begin{align}
% \text{PPL}_M(\mathbf{x}) &= \exp\left(-\frac{1}{T} \sum_{t=1}^{T} \left[\log P_M(x_t | \mathcal{L}_t, \mathcal{S}_t) + \log P_M(\mathcal{L}_t | \mathbf{x_{<t}}) + \log P_M(\mathcal{S}_t | \mathbf{x_{<t}})\right]\right) \nonumber\\
% &= \text{PPL}_{\text{local}}(\mathbf{x}) \cdot \text{PPL}_{\text{syntax}}(\mathbf{x}) \cdot \text{PPL}_{\text{semantic}}(\mathbf{x}) \label{eq:ppl_decomposition}
% \end{align}

% where each component measures distinct model capabilities:

% \textbf{Local Prediction Capability} ($\text{PPL}_{\text{local}}$): Measures the model's ability to predict immediate token sequences based on short-range dependencies and statistical patterns.

% \textbf{Syntactic Understanding} ($\text{PPL}_{\text{syntax}}$): Captures the model's grasp of grammatical structures, part-of-speech consistency, and syntactic well-formedness.

% \textbf{Semantic Coherence} ($\text{PPL}_{\text{semantic}}$): Reflects the model's capacity for maintaining topical consistency, logical reasoning, and long-range discourse coherence.

% This decomposition justifies the use of perplexity as a metric for model collapse: dramatic increases in PPL reflect fundamental breakdowns in core language modeling capabilities, which cascade to impair performance across all downstream tasks that depend on these linguistic foundations. The exponential nature of perplexity amplifies even localized capability losses, making it highly sensitive to critical neuron disruptions.

% \subsection{Neuron Intervention Protocol}

% We employ a masking-based intervention strategy to assess neuron criticality \citep{Meng2022}. For a target neuron $i$ in layer $l$, the masking operation is defined as:

% \begin{equation}
% \tilde{n}_l^{(i)}(\mathbf{x}) = \begin{cases}
% 0 & \text{if neuron } (l, i) \text{ is masked} \\
% n_l^{(i)}(\mathbf{x}) & \text{otherwise}
% \end{cases}
% \end{equation}

% Let $M^{-S}$ denote the model with neuron set $S$ masked, where $S = \{(l_1, i_1), (l_2, i_2), \ldots\}$ represents the collection of masked neurons specified by their layer and index positions.

% \subsection{Model Collapse Definition}

% We define model collapse based on catastrophic performance degradation induced by minimal neuron disruptions. Following the framework established in recent work on model collapse \citep{dohmatob2025strong}, we characterize model collapse through the following mathematical formulation:

% \begin{definition}[Model Collapse via Critical Neuron Disruption]
% \label{def:model_collapse}
% Given a language model $M$ and an input sequence $\mathbf{x} = (x_1, x_2, \ldots, x_T)$, let $M^{-S}$ denote the model with neuron set $S = \{(l_1, i_1), (l_2, i_2), \ldots\}$ masked according to the protocol in Equation~(2).

% Model collapse occurs when there exists an ultra-sparse critical neuron set $S^*$ such that:
% \begin{align}
% \Delta(\mathbf{x}, S^*) &= \log_{10}\left(\frac{\text{PPL}_{M^{-S^*}}(\mathbf{x})}{\text{PPL}_M(\mathbf{x})}\right) \geq \epsilon \nonumber\\
% |S^*| &\ll |N|
% \end{align}
% where $\epsilon > 0$ is a threshold parameter, $|S^*|$ denotes the cardinality of the critical neuron set, and $|N|$ represents the total number of neurons in the model.
% \end{definition}

% \begin{definition}[Minimal Critical Set]
% \label{def:minimal_critical}
% A critical neuron set $S^*$ is minimal if it satisfies the collapse criterion in Equation~(3) while ensuring that no proper subset $S' \subset S^*$ satisfies this condition.
% \end{definition}

% Based on Definition~\ref{def:model_collapse} and Definition~\ref{def:minimal_critical}, we now proceed to design systematic algorithms for identifying critical neurons in LLMs.
